Uncertainty-aware Label Distribution Learning for Facial Expression Recognition

Despite significant progress over the past few years, ambiguity is still a key challenge in Facial Expression Recognition (FER). It can lead to noisy and inconsistent annotation, which hinders the performance of deep learning models in real-world scenarios. In this paper, we propose a new uncertainty-aware label distribution learning method to improve the robustness of deep models against uncertainty and ambiguity. We leverage neighborhood information in the valence-arousal space to adaptively construct emotion distributions for training samples. We also consider the uncertainty of provided labels when incorporating them into the label distributions. Our method can be easily integrated into a deep network to obtain more training supervision and improve recognition accuracy. Intensive experiments on several datasets under various noisy and ambiguous settings show that our method achieves competitive results and outperforms recent state-of-the-art approaches. Our code and models are available at https://github.com/minhnhatvt/label-distribution-learning-fer-tf.

==> 4_methodology.tex <==
\section{Introduction}
\label{sec:intro}
Facial expression recognition (FER) plays an important role in understanding people's feelings and interactions between humans. Recently, automatic emotion recognition has gained a lot of attention from the research community~\cite{academia_industry} due to its applications in healthcare~\cite{application_health_care}, surveillance~\cite{application_surveillance}, or human-robot interaction~\cite{application_hci}. Most recent FER methods utilize deep learning~\cite{cnn} and achieve better results than handcrafted features approaches \cite{hog,lbp}. The success of deep networks can be attributed to large-scale FER datasets such as AffectNet \cite{affectnet}, EmotioNet \cite{emotionet}, and RAF-DB \cite{raf_db}. Some datasets describe emotion in terms of Action Units (AUs) following the Facial Action Coding System \cite{facs} or quantifying affection over continuous scales such as valence and arousal \cite{dim_model} while most of them classify facial expressions into basic universal emotions \cite{6emotions,contempt} and the neutral state.
% including \texttt{anger}, \texttt{disgust}, \texttt{fear}, \texttt{happiness}, \texttt{sadness}, \texttt{surprise},  \texttt{neutral} \cite{6emotions}, and \texttt{contempt} \cite{contempt}. 

Unfortunately, large-scale FER datasets often suffer from the problem of label uncertainty and annotation ambiguity \cite{ipa2lt,ldl_alsg,dmue}. People with different backgrounds might perceive and interpret facial expressions differently, which can lead to inconsistent and uncertain labels \cite{ipa2lt,dmue}. In addition, real-life facial expressions usually manifest a mixture of feelings \cite{edl,ldl_alsg} rather than a single exaggerated emotion often found in the lab-controlled setting.
For example, Figure~\ref{fig:motivation} shows that people may have different opinions about the expressed emotion, particularly in ambiguous images. We argue that distribution over emotion categories is better than a single label because it takes all sentiment classes into account and can cover various interpretations, thus mitigating the effect of ambiguity. However, most current large-scale FER datasets only provide a single label for each sample instead of a label distribution, which means we do not have a comprehensive description for each facial expression. This can lead to a lack of supervision during training and pose a big challenge for many FER systems.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/motivation.pdf}
    \caption{
    % \vspace{-2ex}
    User study results by 50 volunteers on three random images from RAF-DB dataset. The expression on the right image are more ambiguous, which leads to high uncertainty in emotion labels. Labels at the bottom denote the provided annotation from the dataset. (Su=\texttt{Surprise}, Fe=\texttt{Fear}, Di=\texttt{Disgust}, Ha=\texttt{Happy}, Sa=\texttt{Sad}, An=\texttt{Angry}, Ne=\texttt{Neutral})
    %Also, a single-label provided may not  cover sufficient emotional information to train a neural network model efficiently.
    }
    \vspace{-3ex}
    \label{fig:motivation}
\end{figure*}

To overcome annotation ambiguity in facial expression recognition, 
this paper proposes a new uncertainty-aware label distribution learning method that constructs emotion distributions for training samples. Specifically, for each training instance, we leverage the valence-arousal information to identify a set of neighbors and calculate their corresponding contributions using our adaptive similarity mechanism. We then aggregate neighborhood information with the provided single label, adjusted by its uncertainty factor, to generate the target label distribution. Finally, we use the constructed distribution as supervision signals to optimize the model via label distribution learning. We also introduce a discriminative loss that reduces intra-class variations and encourages inter-class differences to improve the model's robustness against ambiguous features. Note that the distribution construction only occurs during training while the inference process remains intact. 
% The extensive experiments show that our method outperforms recent state-of-the-arts and achieves competitive results, both quantitatively and qualitatively. 
In summary, our contributions are as follows:
\begin{enumerate}
    \item We propose a new label distribution learning method for FER under ambiguous label conditions by exploiting the neighborhood information in the valence-arousal space.  
    % Our method can be easily integrated into existing networks to improve their robustness against ambiguity without introducing extra computation costs to inference.
    % without changing the backbone.
    % The target label distribution is constructed with the assistance of valence-arousal space.
    \item Our uncertainty-aware label distribution construction can provide more accurate and richer supervision for training deep FER networks, allowing them to learn from ambiguous data effectively in an end-to-end manner. 
    % \item To combat against ambiguous features, a modification of center loss is designed to enhance the learned representations by reducing intra-class variations and increasing inter-class differences.
    \item We perform extensive experiments under various synthetic and real-world ambiguity settings and achieve state-of-the-art results on RAF-DB, AffectNet, and SFEW datasets. Our source code and pretrained models will be released for further study.    
\end{enumerate}



==> draft.tex <==
%%% Introducing LDL as method for addressing label ambiguity and inconsistency compared with prior methods \cite{deepldl}

% The general label distribution learning framework is divided into two main stages: the first stage is to construct the target label distribution and the second is to fit the model from that distribution. 

%BEGIN_FOLD
% \subsection{Multi-task Label Distribution Learning}
% Our work generalizes the method proposed by Cipolla \etal \cite{mtl_uncertainty_weigh_loss} in a Label Distribution Learning manner

% We denote $f(\mathbf{x}; \mathbf{\theta}) $ as the output of the network with respect to the input $\mathbf{x}$, the network is parameterized by 
% $\mathbf{\theta}$.

% \textbf{LDL for regression task.}
% For many regression tasks, it is reasonable to assume the output and target label are normal distributed. Let  $\mathbf{\hat{y}}$ and $\mathbf{y}$ be the network's prediction and true label distribution. We have:
% \begin{align*}
%     \hat{y} \sim \mathcal{N}(\hat{\mu},\,\hat{\sigma}^{2}) &&
%     y \sim \mathcal{N}(\mu,\sigma^{2})
% \end{align*}
% If the Kullback-Leibler (KL) divergence is
% used to measure the distance between the true and predicted distribution, than we want to minimize the following loss function:
% \begin{align*}
%     \mathbf{D_{KL}} \left(y \middle\| \hat{y} \right) &= \mathbf{D_{KL}} \left(\mathcal{N}(\mu,\sigma^{2}) \middle\| \mathcal{N}(\hat{\mu},\,\hat{\sigma}^{2}) \right) \\
%     &=  \int_{z}{y(z)\left[ \log{y(z)} - \log{\hat{y}(z)} \right]dz}\\
%     &= \int{ y(z)\left[\log{\frac{\hat{\sigma}}{\sigma} +\frac{1}{2} \left( (\frac{z-\hat{\mu}}{\hat{\sigma}})^{2} - (\frac{z-\mu}{\sigma})^{2} \right)} \right]dz}\\
%     &= \EX_{z \sim y(z)} \left[\log{\frac{\hat{\sigma}}{\sigma} +\frac{1}{2} \left( (\frac{z-\hat{\mu}}{\hat{\sigma}})^{2} - (\frac{z-\mu}{\sigma})^{2} \right)} \right\\
%     &= \log{\frac{\hat{\sigma}}{\sigma}} + \frac{1}{2\hat{\sigma}^2}\EX_{z \sim y(z)}\left[(z-\hat{\mu})^2 \right] 
%     - \frac{1}{2\sigma^2}\EX_{z \sim y(z)} \left[ (z-\mu)^2\right]\\ 
%     &= \log{\frac{\hat{\sigma}}{\sigma}} + \frac{1}{2\hat{\sigma}^2}\EX_{z \sim y(z)}\left[z^2-2z\hat{\mu} + \hat{\mu}^2 \right] - \frac{1}{2}\\
%     &= \log{\frac{\hat{\sigma}}{\sigma}} + \frac{1}{2\hat{\sigma}^2}\left[\sigma^2 + (\mu -\hat{\mu})^2 \right] - \frac{1}{2} \\
%     &= \left[\frac{1}{2\hat{\sigma}^2}(\mu - \hat{\mu})^2 + \log{\hat{\sigma}}\right] + \frac{\sigma}{2\hat{\sigma}^2} + \log{\sigma} - \frac{1}{2}
% \end{align*}
% Notice that when $\hat{\sigma}$ is proportional to $\sigma$, i.e., $\hat{\sigma} \propto \sigma$, the KL Divergence Loss function above becomes the objective function (Eq.7) proposed in \cite{mtl_uncertainty_weigh_loss}

% \textbf{LDL for classification task.}
% Here we consider the general case where the output and the target follow Gibbs distribution:
% \begin{align*}
%     \hat{y}_i \propto \exp{\frac{\bar{f}_i(\mathbf{x}; \mathbf{\theta})}{\hat{\sigma}^2}} && 
%     y_i \propto \exp{\frac{\bar{y}_i}{\sigma^2}}
% \end{align*}
% Where $\bar{f}_i$ and $\bar{y}_i$ are the raw value of state $i$ (pre-activate). 
% To make $\hat{y}$ and $y$ valid distribution, i.e., $\sum_{i}y_i = 1$
% (the total probability across all state must sum to 1). We normalize them by applying softmax function:
% \begin{align*}
%     \hat{y} = softmax(\frac{\bar{f}(\mathbf{x}; \mathbf{\theta})}{\hat{\sigma}^2}) && y = softmax(\frac{\bar{y}}{\sigma^2})
% \end{align*}

% The KL Divergence loss between $\hat{y}$ and $y$:
% \begin{align*}
%     \mathbf{D_{KL}} \left(y \middle\| \hat{y} \right) &=
%     \sum_{i=1}^K\left[y_i\log{y_i} - y_i\log{\hat{y}_i}\right]\\
%     &= \mathcal{H}(y, \hat{y}) - \mathcal{H}(y)
% \end{align*}
% Optimizing the loss function above w.r.t $\theta$ is equal to minimizing the cross-entropy loss between $\hat{y}$ and $y$:
% \begin{align*}
%     \mathcal{H}(y, \hat{y}) &= \sum_{i=1}^Ky_i\log{\left[\sum_{c=1}^K\exp(\frac{\bar{f}_c(\mathbf{x}; \mathbf{\theta})}{\hat{\sigma}^2})\right]} - \sum_{i=1}^K y_i\frac{\bar{f}_i(\mathbf{x};\mathbf{\theta})}{\hat{\sigma}^2}\\
%     &= log{\left[\sum_{c=1}^K\exp(\frac{\bar{f}_c(\mathbf{x}; \mathbf{\theta})}{\hat{\sigma}^2})\right]} - \frac{1}{\hat{\sigma}^2}\sum_{i=1}^Ky_i\bar{f}_i(\mathbf{x};\mathbf{\theta})\\
%     &= log{\left[\sum_{c=1}^K \Big(\exp(\bar{f}_c(\mathbf{x}; \mathbf{\theta})) \Big)^{\frac{1}{\hat{\sigma}^2}}\right]} - \frac{1}{\hat{\sigma}^2}\sum_{i=1}^Ky_i\bar{f}_i(\mathbf{x};\mathbf{\theta})
% \end{align*}
% With the assumption relaxation as in \cite{mtl_uncertainty_weigh_loss}, i.e., $\log\sum_{c=1}^K \Big(\exp(\bar{f}_c(\mathbf{x}; \mathbf{\theta})) \Big)^{\frac{1}{\hat{\sigma}^2}} \approx \\ \log\hat{\sigma} \Big(\sum_{c=1}^K \exp(\bar{f}_c(\mathbf{x}; \mathbf{\theta})) \Big)^{\frac{1}{\hat{\sigma}^2}}$, we will obtain the same multi-task loss function proposed in \cite{mtl_uncertainty_weigh_loss}:
% \begin{align*}
%     -\frac{1}{\hat{\sigma}^2}\sum_{i=1}^{K}y_i\log{\hat{y}_i} + \log{\hat{\sigma}}
% \end{align*}%%%
%END_FOLD

==> tmp.tex <==
\subsection{Experiments with Noisy Labels}
% \begin{table*}[h]
% \centering
% \caption{Test accuracy of different methods with synthetic noise. (TBD)\strut}
%     \setlength\aboverulesep{0pt}\setlength\belowrulesep{0pt}
%     \setcellgapes{3pt}\makegapedcells
%     \setlength{\tabcolsep}{6.5pt} % Default value: 6pt
    
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{r|l|ccc|ccc} 
%     \hline
%     \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Noise\\ ratio\end{tabular}}} & \multicolumn{1}{c|}{\multirow{3}{*}{Method}} & \multicolumn{6}{c}{Accuracy (\%)} \\ 
%     \cline{3-8}
%     \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{Symmetric noise} & \multicolumn{3}{c}{Asymmetric noise} \\ 
%     \cline{3-8}
%     \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & RAF-DB & AffectNet & SFEW & RAF-DB & AffectNet & SFEW \\ 
%     \hline
%     \multirow{3}{*}{10\%} & ResNet18 \cite{resnet} & 82.08 & 62.13 & 48.83 & 82.70 & 62.20 & 48.45 \\
%      & SCN \cite{scn} & 84.19 & - & - & 83.93 & - & - \\
%      & LDLVA (ours) & \textbf{85.69} & \textbf{63.17} & \textbf{52.58} & \textbf{86.24} & \textbf{63.32} & \textbf{53.92} \\ 
%     \hline
%     \multirow{3}{*}{20\%} & ResNet18 \cite{resnet} & 80.65 & 60.73 & 42.58 & 80.80 & 60.86 & 44.54 \\
%      & SCN \cite{scn} & 82.01 & - & - & 82.66 & - & - \\
%      & LDLVA (ours) & \textbf{83.90} & \textbf{62.47} & \textbf{49.35} & \textbf{84.35} & \textbf{62.80} & \textbf{50.13} \\ 
%     \hline
%     \multirow{3}{*}{30\%} & ResNet18 \cite{resnet} & 78.92 & 57.42 & 38.96 & 79.13 & 58.99 & 39.68 \\
%      & SCN \cite{scn} & 80.22 & - & - & 80.93 & - & - \\
%      & LDLVA (ours) & \textbf{82.95} & \textbf{59.79} & \textbf{45.74} & \textbf{83.28} & \textbf{61.31} & \textbf{47.22} \\ 
%     \hline
%     \multirow{3}{*}{40\%} & ResNet18 \cite{resnet} & 76.51 & 56.24 & 35.24 & 77.26 & 56.92 & 35.59 \\
%      & SCN \cite{scn} & 78.26 & - & - & 78.88 & - & - \\
%      & LDLVA (ours) & \textbf{80.57} & \textbf{58.35} & \textbf{43.20} & \textbf{81.35} & \textbf{59.33} & \textbf{43.67} \\
%     \hline
%     \end{tabular}%
%     }
%     \label{table:noise_result}
% \end{table*}

\begin{table}[h]
\centering
\caption{Test accuracy of different methods with synthetic noise \strut}
    \setlength\aboverulesep{0pt}\setlength\belowrulesep{0pt}
    \setcellgapes{3pt}\makegapedcells
    \setlength{\tabcolsep}{6.5pt} % Default value: 6pt
    
    % \resizebox{\textwidth}{!}{%
    \resizebox{\textwidth}{!}{
    \begin{tabular}{r|l|ccc} 
    \hline
    \multirow{2}{*}{
        \begin{tabular}[c]{@{}c@{}}
            Noise\\ 
            ratio
        \end{tabular}
    } & \multirow{2}{*}{Method} & \multicolumn{3}{c}{Accuracy (\%)} \\
	\cmidrule{3-5}

	& & RAF-DB & AffectNet & SFEW \\
	\midrule
	\midrule

    \multirow{4}{*}{10\%} 
     & Baseline & 83.28 $\pm$ 0.45 & 60.14 $\pm$ 0.23 & 45.98 $\pm$ 0.93 \\
     & SCN \cite{scn} & 84.65 $\pm$ 0.32 & 61.57 $\pm$ 0.15 & 49.51 $\pm$ 0.76  \\
     & RUL \cite{rul} & 86.24 $\pm$ 0.22 & 62.89 $\pm$ 0.13 & 47.82 $\pm$ 1.32\\
     & LDLVA (ours) & \textbf{87.98 $\pm$ 0.10} & \textbf{64.37  $\pm$ 0.11} & \textbf{53.33 $\pm$ 0.57}  \\ 
    \midrule
    \multirow{4}{*}{20\%} 
     & Baseline & 81.89 $\pm$ 0.61 & 58.37 $\pm$ 0.35 & 41.25 $\pm$ 1.12 \\
     & SCN \cite{scn} & 83.21 $\pm$ 0.49 & 60.83 $\pm$ 0.19 & 46.26 $\pm$ 1.24 \\
     & RUL \cite{rul} & 84.49 $\pm$ 0.24 & 61.74 $\pm$ 0.18 & 44.78 $\pm$ 1.04\\ 
     & LDLVA (ours) & \textbf{86.81 $\pm$ 0.12} & \textbf{63.89 $\pm$ 0.14} & \textbf{51.53 $\pm$ 0.92}  \\ 
    \midrule
    \multirow{4}{*}{30\%} 
     & Baseline & 78.92 $\pm$ 0.59 & 56.94 $\pm$ 0.43 & 38.51 $\pm$ 1.69  \\
     & SCN \cite{scn} & 80.61 $\pm$ 0.54 & 58.80 $\pm$ 0.32 & 43.28 $\pm$ 2.06  \\
     & RUL \cite{rul} & 82.59 $\pm$ 0.42 & 60.77 $\pm$ 0.15 & 41.79 $\pm$ 0.81\\
     & LDLVA (ours) & \textbf{85.85 $\pm$ 0.09} & \textbf{62.57 $\pm$ 0.15} & \textbf{50.3 $\pm$ 0.88}  \\
     
    \bottomrule
    \end{tabular}%
     }
    \label{table:noise_result}
    \vspace{-3ex}
\end{table}
The two main aspects of annotation ambiguity in FER are noisy labels and uncertain visual features \cite{scn}. In particular, it can be difficult for people to accurately recognize the emotions on ambiguous facial images, which can result in noisy and incorrect labels. Therefore, we conduct experiments to study the robustness of our LDLVA on mislabelled data by adding synthetic noise to AffectNet, RAF-DB, and SFEW datasets.
% Due to the inherent ambiguity and uncertainty, people may find it difficult to recognize the facial expression correctly, this leads to the noisy and inconsistent annotations in FER datasets. Therefore, the ability to cope with incorrect labels is critical for a successful FER application.
% To that end, we study the robustness of our approach by conducting experiments on RAF-DB, AffectNet and SFEW datasets, in which label noise is synthetically added. 
More specifically, we randomly flip the labels to one of the other categories. Three levels of noise (10\%, 20\%, 30\% training samples) are studied in our experiment. We quantitatively evaluate our method and compare with the baseline ResNet-18 \cite{resnet} and recent noise-tolerant FER methods including SCN \cite{scn} and RUL \cite{rul}. 

We perform each experiment three times and report the mean accuracy and standard error in Table \ref{table:noise_result}. The results clearly show that our method consistently outperforms other approaches in all cases. Particularly, our model makes significant improvements over the baseline with an average accuracy margin of +5.52\%, +5.13\%, and +9.81\% on the RAF-DB, AffectNet, and SFEW datasets, respectively. We also observe that the improvements are even more apparent when the noise ratio increases, for example, the accuracy improvement on RAF-DB is 4.7\% with 10\% noise and 6.93\% with 30\% noise. 
% This means our method can effectively disambiguate the noisy label and improve the robustness.
% Moreover, compared to the second best method RUL \cite{rul}, our approach also gains an average improvement of +2.44\%, +1.81\% accuracy across the RAF-DB and AffectNet dataset. Another finding is that RUL \cite{rul} perform worse than SCN \cite{scn} on the SFEW dataset. The reason might be that in RUL training strategy, the network is enforced to recognize the right classes from the mixed representation of a facial image pair. This may not be well suited for small dataset like SFEW since the data is insufficient to learn the pairwise relationship of two different categories. 
The consistent results under various settings demonstrate the ability of our method to effectively deal with noisy annotation, which is crucial in the robustness against label ambiguity. 

\subsection{Experiments with Inconsistent Labels}

\begin{table}

\centering
    % make the vertical line continuos
    \setlength\aboverulesep{0pt}\setlength\belowrulesep{0pt}
    \setcellgapes{3pt}\makegapedcells
    \setlength{\tabcolsep}{6.5pt}  % Default value: 6pt

     \resizebox{\textwidth}{!}{
     \begin{tabular}{l|ccc|c} 
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{4}{c}{Accuracy (\%)} \\
	\cmidrule{2-5}
     & AffectNet & RAF-DB & SFEW & Average \\ 
    \midrule
    \midrule
    % Baseline \cite{ldl_alsg} & 57.97 & 81.81 & 52.19 & 63.99 \\
    AIR \cite{air} & 54.23 & 67.37 & 49.88 & 57.16 \\
    NAL \cite{nal} & 55.97 & 84.22 & {58.13} & 66.11 \\
    IPA2LT \cite{ipa2lt} & 57.85 & 83.80 & 53.15 & 64.93 \\
    LDL-ALSG \cite{ldl_alsg} & 58.29 & 85.33 & 55.87 & 66.50 \\ 
    \midrule
    % {LDLVA} (ours) & \textbf{62.89} & \textbf{87.26} & 56.61 & \textbf{68.92} \\ 
    {LDLVA} (ours) & \textbf{60.12} & \textbf{87.26} & \textbf{58.7} & \textbf{68.69}\\
    \bottomrule
    \end{tabular}%
    }
    \caption{Test accuracy of different methods with inconsistent labels %Results of previous methods are taken from \cite{ldl_alsg}.
    \strut}
    \label{tab:cross_dataset_result}
\end{table}


\begin{table}
	\centering
    \setlength\aboverulesep{0pt}\setlength\belowrulesep{0pt}
    \setcellgapes{3pt}\makegapedcells
    
    \setlength{\tabcolsep}{6.5pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cc|cc} 
    % \begin{tabular}{ccc|cc} 
    \toprule
    \begin{tabular}[c]{@{}c@{}}Adaptive\\similarity~\end{tabular} & \begin{tabular}[c]{@{}c@{}}Valence-arousal\\value~\end{tabular} &
    % w/W & w/gVA &
    \begin{tabular}[c]{@{}c@{}}AffectNet\\(original)~\end{tabular} & \begin{tabular}[c]{@{}c@{}}AffectNet\\(30\% noise)\end{tabular} \\ 
    \midrule
    \midrule
    - & pseudo & 63.95 & 60.52 \\ 
    \cmark & pseudo & 65.45 & 62.23 \\ 
    \cmark & groundtruth & 65.74 & 62.57 \\    
    % \xmark & \xmark & 63.95 & 60.52 \\ 
    % \cmark & \xmark & 65.45 & 62.23 \\ 
    % \cmark & \cmark & 65.79 & 62.47 \\
    \bottomrule
    \end{tabular}
    }
    \caption{Performance of our LDLVA on AffectNet dataset with pseudo vs. groundtruth valence-arousal} 
    \label{table:ablation_pseudova}
\vspace{-3ex}
\end{table}


Due to the ambiguous nature of facial expressions, different individuals can assign different labels for the same image as illustrated in Figure \ref{fig:motivation}. Since the annotations for large-scale FER data are commonly obtained via crowd-sourcing, this can create label inconsistency, especially between different datasets. Therefore, to examine the effectiveness of the proposed methods in dealing with this problem, we follow the cross-dataset protocol in previous state-of-the-art methods \cite{ldl_alsg,ipa2lt} and adopt the experimental settings as proposed in \cite{ldl_alsg} for a fair comparison. 
Specifically, the model is trained using the joint training dataset from  RAF-DB and AffectNet. The resulting model is then tested on all three RAF-DB, AffectNet, and SFEW datasets.

% \begin{table}
% \centering
%     % make the vertical line continuos
%     \setlength\aboverulesep{0pt}\setlength\belowrulesep{0pt}
%     \setcellgapes{3pt}\makegapedcells
%     \setlength{\tabcolsep}{6.5pt}  % Default value: 6pt
    
%     \caption{Test accuracy of different methods with inconsistent labels. %Results of previous methods are taken from \cite{ldl_alsg}.
%     \strut}
%     \begin{tabular}{l|ccc|c} 
%     \toprule
%     \multirow{2}{*}{Method} & \multicolumn{4}{c}{Accuracy (\%)} \\
% 	\cmidrule{2-5}
%      & AffectNet & RAF-DB & SFEW & Average \\ 
%     \midrule
%     \midrule
%     % Baseline \cite{ldl_alsg} & 57.97 & 81.81 & 52.19 & 63.99 \\
%     AIR \cite{air} & 54.23 & 67.37 & 49.88 & 57.16 \\
%     NAL \cite{nal} & 55.97 & 84.22 & {58.13} & 66.11 \\
%     IPA2LT \cite{ipa2lt} & 57.85 & 83.80 & 53.15 & 64.93 \\
%     LDL-ALSG \cite{ldl_alsg} & 58.29 & 85.33 & 55.87 & 66.50 \\ 
%     \midrule
%     % {LDLVA} (ours) & \textbf{62.89} & \textbf{87.26} & 56.61 & \textbf{68.92} \\ 
%     {LDLVA} (ours) & \textbf{60.12} & \textbf{87.26} & \textbf{58.7} & \textbf{68.69}\\
%     \bottomrule
%     \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}
%     \end{tabular}%
%     \label{tab:cross_dataset_result}
% \end{table}

Table \ref{tab:cross_dataset_result} reports the results of our experiments. 
Our method achieves the best performance on all three datasets and the highest average accuracy. Notably, LDLVA surpasses the current state-of-the-art LDL-ALSG \cite{ldl_alsg} with an improvement of +2.42\% accuracy. Compared to our approach, LDL-ALSG only uses the neighbors' distributions to constrain the network prediction without constructing a label distribution for the center instance. It also lacks a mechanism to adaptively measure the contribution of each neighbor and the uncertainty of the provided annotation. 
The favorable performance confirms the advantages of our method over previous works and demonstrates the generalization ability to data with label inconsistency, which is essential for real-world FER applications.

\subsection{Experiments on Original Datasets}
\label{sec:exp_original}
\begin{table*}
\small
	\centering
    \caption{Test accuracy of different methods on original datasets \strut} 
    \label{table:clean_data_result}
    % \vspace{1ex}
    % \hfill
    \begin{subtable}[h]{0.3\textwidth}
        \centering
        \caption{AffectNet}
        \begin{tabular}{l  c}
            Method & Acc. (\%) \\
            \hline \hline
            IPFR \cite{IPFR} & 57.40\\
            gaCNN \cite{gacnn} & 58.78   \\
            CAKE \cite{cake} & 61.70 \\
            DDA \cite{dda_loss} & 62.34   \\
            Center loss \cite{center_loss} & 64.09   \\
            % DMUE \cite{dmue} & 62.84 \\       
            % MA-Net \cite{MANet} & 64.53  \\
            % DMUE \cite{dmue} & 63.11 \\
            DACL \cite{dacl_net} & 65.20  \\
            \midrule
            %ResNet18 Vanilla & 60.53 \\
            {LDLVA} (ours) & \textbf{65.74} \\
            % {LDLVA} (ours) & \textbf{66.23}          
      \end{tabular}
      \label{tab:clean_affnet}
    \end{subtable}
    % \hfill
    \hspace{0.5em}
    \begin{subtable}[h]{0.3\textwidth}
        \centering
        \caption{RAF-DB}
        \begin{tabular}{l  c}
            Method & Acc. (\%) \\
            \hline \hline
            gaCNN \cite{gacnn} & 85.07 \\
            RAN	\cite{ran} & 86.90 \\
            SCN \cite{scn}	& 87.03 \\
            DACL \cite{dacl_net} & 87.78 \\
            % MA-Net \cite{MANet} & 88.40 \\
            DMUE \cite{dmue} & 88.76 \\
            RUL	\cite{rul} & 88.98 \\
            % DMUE \cite{dmue} & 89.42 \\
            \midrule
            %ResNet18 Vanilla & 86.27 \\
            {LDLVA} (ours) & \textbf{89.57} \\
            % {LDLVA} (ours) & \textbf{90.35}          
      \end{tabular}
      \label{tab:clean_rafdb}
    \end{subtable}
    % \hfill
    \hspace{0.25em}
    \begin{subtable}[h]{0.3\textwidth}
        \centering
        \caption{SFEW}
        \begin{tabular}{l  c}
            Method & Acc. (\%) \\
            \hline \hline
            Island Loss \cite{island_loss}	& 52.52 \\
            IACNN \cite{iacnn} & 54.30 \\
            IPFR \cite{IPFR} & 55.10 \\
            MultiCNNs\cite{multicnns} & 55.96\\
            RAN	\cite{ran} & 56.40 \\
            DMUE \cite{dmue} & 57.12 \\
            % Cov. Pooling \cite{cov_pooling} & 58.14 \\            
            % DMUE \cite{dmue} & 58.34 \\
            % MA-Net \cite{MANet}	& 59.40 \\
            \midrule
            %ResNet18 Vanilla & 51.29 \\
            {LDLVA} (ours) & \textbf{58.39} \\
            % {LDLVA} (ours) & \textbf{59.90}         
      \end{tabular}
      \label{tab:clean_sfew}
    \end{subtable}
    \vspace{-4ex}
\end{table*}

We further perform experiments on the original AffectNet, RAF-DB, and SFEW to evaluate the robustness of our method to the uncertainty and ambiguity that unavoidably exists in real-world FER datasets. We compare the proposed LDLVA with several state-of-the-art methods in Table \ref{table:clean_data_result}. 
By leveraging label distribution learning on valence-arousal space, our model outperforms other methods and achieves state-of-the-art performance on AffectNet, RAF-DB, and SFEW. Although these datasets are considered to be ``clean", the results suggest that they indeed suffer from uncertainty and ambiguity.
% In addition, to demonstrate that our method can be easily integrated into existing networks, we provide the results corresponding to different backbone architectures in the supplementary. 

\subsection{Qualitative Analysis}
\textbf{Real-world Ambiguity.} To understand more about real-world ambiguous expressions, we conducted a user study with 50 participants who were asked to choose the most clearly expressed emotion on random test images from RAF-DB and AffectNet. The numbers of votes per class are normalized to obtain the emotion distribution. We compare our model's predictions with the survey results in Figure \ref{fig:model_prediction_vs_survey}.
% The normalized result indicates the probability or the importance degree of each emotion presented in each image. 
% In Figure \ref{fig:model_prediction_vs_survey}, We compare the predicted outputs of our LDLVA model and the survey results. \textit{More qualitative results can be found in the supplementary material}.
We can see that these images are ambiguous as they express a combination of different emotions, hence the participants do not fully agree and have different opinions about the most prominent emotion on the faces. 
% Qualitatively, we observe that ambiguities exist in those images. These ambiguities may exhibit difficulties for people in determining the correct emotion, as we can see the participants do not fully agree with each other. 
It is further shown that LDLVA can give consistent results and agree with the perception of humans to some degree, which suggests that our model can effectively address the ambiguity problem in facial expression. 

\begin{figure*}[ht]
    \centering
    \vspace{-1ex}
    \includegraphics[width=0.99\textwidth]{figs/model_vs_survey.pdf}
    \caption{
    Comparison of the results from our survey and our model}
        \vspace{-2ex}
    \label{fig:model_prediction_vs_survey}
\end{figure*}
%\vspace{-3ex} ## no use

\begin{figure*}[!ht]
    \centering
    %\vspace{-3ex}
    \includegraphics[width=0.96\textwidth]{figs/visualize_weighting.pdf}
    \caption{The calibration scores of neighbor images with respect to the main instance. The large image on the left is the main instance. The neighbor images are shown at the top, and their corresponding scores are shown at the bottom}
    \label{fig:visualize_weighting}
    \vspace{-1ex}
\end{figure*}

\textbf{Adaptive Similarity.} Figure \ref{fig:visualize_weighting} presents the normalized {calibration scores} of different neighbors with respect to the center instance computed by our adaptive similarity mechanism. It can be seen that some neighbors may look visually similar to the central image but do not express the same emotion. By giving low calibration values, our method can effectively suppress the negative influence of these neighbors and lower their importance, hence resulting in a more robust and accurate estimation of the emotion distribution. 
% On the other hand, the Weighting Module does not completely omit the contribution of these neighbors. % Since they share similar characteristics with the central image, the model can utilize that information to learn more robust features. 

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.96\textwidth]{figs/visualize_dist_2.pdf}
    \caption{Examples of the emotion distribution recovered by our method when the dataset is contaminated with noisy labels. The label on top of each image is the synthetic noisy label and the bottom denotes the human annotation}
    \label{fig:visualize_dist}
\end{figure*}

\textbf{Constructed Label Distribution.} %To further investigate the effectiveness of our framework in addressing the ambiguity problem in emotion recognition, 
In Figure \ref{fig:visualize_dist}, we visualize the emotion distributions reconstructed by our method on mislabelled images. Despite the incorrect annotations, our approach is able to construct plausible distributions and discover the correct labels. It is also noteworthy that some expressions manifest multiple emotions rather than only the single provided category, which means the discovered distribution can provide more supervision for training. 
% Furthermore, we can observe that ambiguity exists in these images. For instance, the facial images are mixed with multiple expressions and a single discrete label is insufficient to represent these emotions. %As a consequence, these weaknesses may hinder the FER performance and other related emotion analysis tasks. 
% We can see that it is not a trivial task to quantify the emotion of these images correctly. The qualitative results show that our method is not only robust to the noisy label but is also able to handle the ambiguity problem in FER.

\begin{figure}[!ht]
    \centering
    \vspace{-2ex}
    \includegraphics[width=0.96\textwidth]{figs/uncertainty.pdf}
    \caption{
    Visualization of uncertainty values of some examples from RAF-DB dataset. %Each image is tagged with its estimated uncertainty values and the original label. 
    High uncertainty value means that the model is uncertain about the label of an image and vice versa}
    \label{fig:uncertainty}
\end{figure}
%\vspace{-3ex}

\textbf{Uncertainty Factor.} 
% We further qualitatively investigate our method under the uncertainties that inevitably exists in real-world FER datasets. 
Figure \ref{fig:uncertainty} shows the estimated uncertainty factors of some training images in the RAF-DB dataset and their original labels. The uncertainty values decrease from top to bottom. Highly uncertain labels can be caused by low-quality inputs (as shown in \texttt{Angry} and \texttt{Surprise} columns) or ambiguous facial expressions. In contrast, when the emotions can be easily recognized as those in the last row, the uncertainty factors are assigned low values. This characteristic can guide the model to decide whether to put more weights on the provided label or the neighborhood information. Therefore, the model can be more robust against uncertainty and ambiguity.
% In the first row, we visualize images with large uncertainty values. We can see that these uncertainties are attributed to various factors, such as the low-quality images or ambiguous expressions. 
% These factors can lead to inconsistent and noisy annotations, which may potentiality hinder the ability of a FER system if they are not considered properly. In contrast, the facial expressions in the last row are apparently recognizable, which leads to low uncertainty values as the model are more confident about the expression label of these images. These analyses demonstrate the benefits of our uncertainty-aware scheme as it help mitigate the adverse effect of ambiguous data. This can aid the model to appropriately reconstruct the emotion distribution since it is encouraged to pay more attention to the neighbor information.

\subsection{Ablation Study}
% combine ablation analysis and weighting module table into a single analysis
\textbf{Contribution of 
Each Component.} In Table \ref{tab:ablation_study}, we present the accuracy corresponding to different combinations of our components: label distribution (whether to construct $\bm{d}^i$ or not), adaptive similarity (whether to compute calibration scores or directly use local similarity scores as contribution degrees), uncertainty factor (whether to use separate $\lambda^i$ for each instance or share a fixed value $\lambda$ for all training samples), and discriminative loss (whether to incorporate $\mathcal{L}_D$ in Equation \ref{eq:total_loss} or not). By employing label distribution with adaptive similarity \texttt{(ii)}, we can significantly improve the accuracy of the vanilla approach \texttt{(i)} by 1.99\% on original RAF-DB and 3.77\% on 30\%-noise RAF-DB. Further integrating uncertainty factor and discriminative loss consistently boost the performance of the model, as shown in the results of \texttt{(iii)} and \texttt{(v)} respectively. 
%We also note that without adaptive similarity as in \texttt{(iv)}, the accuracy of the model drops from 89.57\% and 85.85\% to 88.52\% and 83.56\% on the original and 30\%-noise RAF-DB. 
The results show the effectiveness of each component as well as the advantages of their combination in our LDLVA method. 

% \begin{table}
% 	\centering
%     \setlength\aboverulesep{0pt}\setlength\belowrulesep{0pt}
%     \setcellgapes{3pt}\makegapedcells
    
%     \setlength{\tabcolsep}{6.5pt} % Default value: 6pt
%     \renewcommand{\arraystretch}{1.5} % Default value: 1
%     \caption{Ablation analysis of different components in our method. \strut} 
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{c|cccc|cc} 
%     \midrule
%     Setting & 
%     \begin{tabular}[c]{@{}c@{}}Label\\distribution~\end{tabular} &
%     \begin{tabular}[c]{@{}c@{}}Adaptive\\similarity~\end{tabular} &    \begin{tabular}[c]{@{}c@{}}Uncertainty\\factor~\end{tabular} &
%     \begin{tabular}[c]{@{}c@{}}Discriminative\\loss~\end{tabular} & 
%     \begin{tabular}[c]{@{}c@{}}RAF-DB\\(original)~\end{tabular} & \begin{tabular}[c]{@{}c@{}}RAF-DB\\(30\% noise)\end{tabular} \\ 
%     \midrule
%     \midrule
%     \texttt{(i)} & - & - & - & - & 86.27 & 78.92 \\ 
%     \midrule
%     \texttt{(ii)} & \cmark & \cmark & - & - & 88.16 & 82.69 \\ 
%     \texttt{(iii)} & \cmark & \cmark & \cmark & - & 89.28 & 84.38 \\    
%     \midrule
%     \texttt{(iv)} & \cmark & - & \cmark & \cmark & 88.52 & 83.56 \\   
%     \texttt{(v)} & \cmark & \cmark & \cmark & \cmark & 89.57 & 85.85 \\     
%     \bottomrule
%     \end{tabular}
%     }
%     \label{table:ablation_study}
%     \vspace{-3ex}
% \end{table}


\begin{table}
\centering
    % make the vertical line continuos
    \setlength\aboverulesep{0pt}\setlength\belowrulesep{0pt}
    \setcellgapes{3pt}\makegapedcells
    \setlength{\tabcolsep}{6.5pt}  % Default value: 6pt
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{c|cccc|cc} 
    \midrule
    Setting & 
    \begin{tabular}[c]{@{}c@{}}LD~\end{tabular} &
    \begin{tabular}[c]{@{}c@{}}AS~\end{tabular} &    \begin{tabular}[c]{@{}c@{}}UF~\end{tabular} &
    \begin{tabular}[c]{@{}c@{}}DL~\end{tabular} & 
    \begin{tabular}[c]{@{}c@{}}RAF-DB\\(original)~\end{tabular} & \begin{tabular}[c]{@{}c@{}}RAF-DB\\(30\% noise)\end{tabular} \\ 
    \midrule
    \midrule
    \texttt{(i)} & - & - & - & - & 86.27 & 78.92 \\ 
    \midrule
    \texttt{(ii)} & \cmark & \cmark & - & - & 88.16 & 82.69 \\ 
    \texttt{(iii)} & \cmark & \cmark & \cmark & - & 89.28 & 84.38 \\    
    \midrule
    \texttt{(iv)} & \cmark & - & \cmark & \cmark & 88.52 & 83.56 \\ 
    \texttt{(v)} & \cmark & \cmark & \cmark & \cmark & 89.57 & 85.85 \\     
    \bottomrule
    \end{tabular}
    }
\caption{Component analysis (LD: Label Distribution, AS: Adaptive Similarity, UF: Uncertainty Factor, DL: Discriminative Loss) \strut}
\label{tab:ablation_study}
\end{table}


\begin{figure}
  {
  \centering
  \includegraphics[width=0.36\textwidth]{figs/ablation_neighbors_2.pdf}
 }
  {\caption{Evaluation results with different numbers of neighbors}\label{fig:ablation_study}}

\end{figure}


% {\textbf{Contribution of each component,}}. \textbf{Need determination for name of each component} In Table \ref{table:ablation_component}, we investigate the effect of the {Distribution}, {Uncertainty-aware} and the {DiscriminativeLoss} on the original RAF-DB and its noisy version with a ratio of 30\%. Since the {Uncertainty-aware} is optimized jointly with the network in our method. To evaluate the it independently (the second row), the uncertainty values $\lambda$ are set as constant based on validation for all samples. 
% To evaluate the {Uncertainty-aware} as a indepedent component (the third row), we apply the same strategy as in \cite{scn} to perform loss weighting with the uncertainty values, instead of training the network with the reconstructed distribution. Note that the uncertainty values are still updated by considering the classification loss $\mathcal{L}_{cls}$. 
% Overall, we observe that the {Distribution} is the most contributed component. In particular, 
% when integrated only the {Distribution} into the backbone network (the second row), it substantially improves the baseline results by 1.99\% on RAF-DB and 3.77\% on RAF-DB with 30\% noise. This verify the effectiveness of the label distribution to disambiguate facial expressions by considering the relative importance of all categories rather than forcing them to be exact single category. Additionally, we find that the {Uncertainty-aware} also plays an important role to enhance the robustness of the model against uncertainties and label noise in FER datasets.  When incorporating these two components, we can further gain an improvement of 1.02\% and achieve 89.29\% accuracy on RAF-DB, comparing to only using the {Distribution}. The {DiscriminativeLoss} can also yield performance gain by a fair margin, which implies that it can help the network learn useful feature to accurately describe the facial image and alleviate the ambiguous among expressions.

% \begin{table}
% 	\centering
%     \setlength\aboverulesep{0pt}\setlength\belowrulesep{0pt}
%     \setcellgapes{3pt}\makegapedcells
    
%     \setlength{\tabcolsep}{6.5pt} % Default value: 6pt
%     % \renewcommand{\arraystretch}{1.5} % Default value: 1
%     \caption{Ablation analysis of different components in our framework. \strut} 
%     \begin{tabular}{ccc|cc} 
  
%     \midrule
%     \begin{tabular}[c]{@{}c@{}}Reconstructing\\distribution~\end{tabular} & \begin{tabular}[c]{@{}c@{}}Trainable\\uncertainty value~\end{tabular} &
%     \begin{tabular}[c]{@{}c@{}}Discriminative\\loss~\end{tabular} & 
%     \begin{tabular}[c]{@{}c@{}}RAF-DB\\(clean)~\end{tabular} & \begin{tabular}[c]{@{}c@{}}RAF-DB\\(30\% noise)\end{tabular} \\ 
%     \midrule
%     \midrule
%     -  & - & - & 86.27 & 78.92 \\ 
%     \cmark & - & - & 88.16 & 82.69 \\ 
%     - & \cmark & - & 87.52 & 81.12 \\
%     - & - & \cmark & 86.86 & 79.97\\
%     \cmark & \cmark & - & 89.28 & 84.38 \\    
%     \cmark & \cmark & \cmark & 89.57 & 85.85 \\   
%     \midrule
%     \end{tabular}
%     \label{table:ablation_component}
% \end{table}

% {\textbf{Weighting Module} Table {\ref{table:ablation_weighting}} shows the performance of different weighting strategies on RAF-DB datasets. \emph{No Weighting} means that we set $b^i_k = 1$ for all neighbors and the contribution degree only depends the local similarity $a^i_k$. The \emph{Self-Attention} operation is similar to the 1-block MLP but it takes only $\bm{v}^k$ as input instead of the concatenated vectors. This table shows that our Weighting Module with MLP blocks clearly outperforms both the Self-Attention and No Weighting mechanisms. Using deeper MLP also helps to improve the results. We recommend using  MLP with 3 blocks in our Weighting Module as the deeper setting requires more computational resources but the performance gain is not significant.}

% ========================== Pseudo valence-arousal groundtruth===========================
\textbf{Pseudo vs. Groundtruth Valence-Arousal.} In Table \ref{table:ablation_pseudova}, we compare the performance of our model when using the pseudo valence-arousal generated by \cite{va_prediction} versus the valence-aroural groundtruth provided in AffectNet dataset. 
% The results show that without Weighting Module, the performance when using the pseudo-valence-arousal is significantly lower than the one using the actual ground-truth. Furthermore, we notice that using the Weighting Module helps improve the accuracy asymptotically to the performance when using the valence-arousal values provided by annotators.
We can see that with pseudo valence-arousal, our adaptive similarity mechanism helps improve the model's accuracy significantly. Furthermore, the adaptive similarity makes the performance when using pseudo valence-arousal comparable with the actual valence-arousal ground-truth. 
The results validate the benefits of our method and alleviate the need for manually annotated valence-arousal.

% \begin{figure}[hbt]
%     \begin{minipage}{0.48\hsize}
%         \includegraphics[width=0.9\hsize]{example-image-c}
%         \captionof{figure}{figure c}
%         \label{fig:c}
%     \end{minipage}
%     \hfill
    
%     \begin{minipage}{0.48\hsize}
    
% 	\centering
%     \caption{Performance of our LDLVA on AffectNet dataset with pseudo vs. groundtruth valence-arousal. \strut} 
%     \vspace{1ex}
%     \setlength\aboverulesep{0pt}\setlength\belowrulesep{0pt}
%     \setcellgapes{3pt}\makegapedcells
%     \resizebox{0.45\textwidth}{!}{%
% 	\begin{tabular}{cc|cc}

%         \toprule
%         \begin{tabular}[c]{@{}c@{}}Weighting\\Module~\end{tabular} & \begin{tabular}[c]{@{}c@{}}Valence-arousal\\Values~\end{tabular} &
%         \begin{tabular}[c]{@{}c@{}}AffectNet\\(clean)~\end{tabular} & \begin{tabular}[c]{@{}c@{}}AffectNet\\(30\% noise)\end{tabular} \\ 
%         \midrule
%         \midrule
%         - & pseudo & 63.95 & 60.82 \\ 
%         \cmark & pseudo & 65.45 & 62.33 \\ 
%         \cmark & groundtruth & 65.74 & 62.57 \\    
%         \bottomrule

% 	\end{tabular}%
% 	}
%     \label{table:ablation_pseudova}
%     \centering
%         \begin{tabular}{ll}
%             \hline
%             column1a & column2a \\
%             column1b & column2b \\
%             column1c & column2c \\
%             \hline
%         \end{tabular}
%         \captionof{table}{table 1}
%         \label{tab:1}
%     \end{minipage}
% \end{figure}

% \begin{table}[h]
% \centering
% \parbox{.45\linewidth}{    
%     \centering
%     \caption{Performance of different weighting strategies on RAF-DB dataset.\strut}
%     \setlength\aboverulesep{0pt}\setlength\belowrulesep{0pt}
%     \setcellgapes{3pt}\makegapedcells
    
%     \resizebox{0.45\textwidth}{!}{%
%     \begin{tabular}{l|cc} 
%     	\toprule
%         \multicolumn{1}{c|}{Weighting strategy} & 
%     	\begin{tabular}[c]{@{}c@{}}RAF-DB\\(clean)\end{tabular} & \begin{tabular}[c]{@{}c@{}}RAF-DB\\(30\% noise)~ ~\end{tabular} \\ 
%     	\midrule
%     	\midrule
%         No Weighting & 88.52 & 83.56 \\ 
%         Self-Attention & 88.88 & 84.17 \\ 
%         Our weighting module & 89.57 & 85.85 \\
%         % Weighting with 1-block MLP & 88.12 & 82.34 \\ 
%         % Weighting with 2-block MLP & 88.4 & 83.41 \\ 
%         % Weighting with 3-block MLP & 88.66 & 83.9 \\ 
%         % Weighting with 4-block MLP & 88.72 & 83.81 \\
%         \bottomrule
%     \end{tabular}%
%     }
%     \label{table:ablation_weighting}
% }
% \qquad
% \parbox{.45\linewidth}{
% 	\centering
%     \caption{Performance of our LDLVA on AffectNet dataset with pseudo vs. groundtruth valence-arousal. \strut} 
%     \vspace{1ex}
%     \setlength\aboverulesep{0pt}\setlength\belowrulesep{0pt}
%     \setcellgapes{3pt}\makegapedcells
%     \resizebox{0.45\textwidth}{!}{%
% 	\begin{tabular}{cc|cc}
	
%         \toprule
%         \begin{tabular}[c]{@{}c@{}}Weighting\\Module~\end{tabular} & \begin{tabular}[c]{@{}c@{}}Valence-arousal\\Values~\end{tabular} &
%         \begin{tabular}[c]{@{}c@{}}AffectNet\\(clean)~\end{tabular} & \begin{tabular}[c]{@{}c@{}}AffectNet\\(30\% noise)\end{tabular} \\ 
%         \midrule
%         \midrule
%         - & pseudo & 63.95 & 60.82 \\ 
%         \cmark & pseudo & 65.45 & 62.33 \\ 
%         \cmark & groundtruth & 65.74 & 62.57 \\    
%         \bottomrule

% 	\end{tabular}%
% 	}
%     \label{table:ablation_pseudova}
% }
% \end{table}

% \begin{table}
% \centering
%     \centering
%     \setlength\aboverulesep{0pt}\setlength\belowrulesep{0pt}
%     \setcellgapes{3pt}\makegapedcells

%     \setlength{\tabcolsep}{6.5pt} % Default value: 6pt
    
%     \caption{Performance of different weighting strategies on RAF-DB dataset.\strut}
%     \begin{tabular}{l|cc} 
% 	\toprule
%     \multicolumn{1}{c|}{Weighting strategy} & 
% 	\begin{tabular}[c]{@{}c@{}}RAF-DB\\(clean)\end{tabular} & \begin{tabular}[c]{@{}c@{}}RAF-DB\\(20\% noise)~ ~\end{tabular} \\ 
% 	\midrule
% 	\midrule
%     No Weighting & 87.61 & 81.61 \\ 
%     Self-Attention & 88.97 & 82.01 \\ 
%     Weighting with 1-block MLP & 88.12 & 82.34 \\ 
%     Weighting with 2-block MLP & 88.4 & 83.41 \\ 
%     Weighting with 3-block MLP & 88.66 & 83.9 \\ 
%     Weighting with 4-block MLP & 88.72 & 83.81 \\
%     \bottomrule
%     \end{tabular}
%     \label{table:ablation_weighting}
% \end{table}

% \begin{table}
% 	\centering
%     \setlength\aboverulesep{0pt}\setlength\belowrulesep{0pt}
%     \setcellgapes{3pt}\makegapedcells
    
%     \setlength{\tabcolsep}{6.5pt}

%     \caption{Performance of our LDLVA on AffectNet dataset with pseudo vs. groundtruth valence-arousal (VA).} %The first two rows illustrate results when using the pseudo-VA instead of the groundtruth values.  \strut} 
%     \begin{tabular}{cc|cc} 
%     % \begin{tabular}{ccc|cc} 
%     \toprule
%     \begin{tabular}[c]{@{}c@{}}Weighting\\Module~\end{tabular} & \begin{tabular}[c]{@{}c@{}}Valence-arousal\\Values~\end{tabular} &
%     % w/W & w/gVA &
%     \begin{tabular}[c]{@{}c@{}}AffectNet\\(clean)~\end{tabular} & \begin{tabular}[c]{@{}c@{}}AffectNet\\(20\% noise)\end{tabular} \\ 
%     \midrule
%     \midrule
%     - & pseudo & 63.95 & 60.52 \\ 
%     \cmark & pseudo & 65.45 & 62.23 \\ 
%     \cmark & groundtruth & 65.79 & 62.47 \\    
%     % \xmark & \xmark & 63.95 & 60.52 \\ 
%     % \cmark & \xmark & 65.45 & 62.23 \\ 
%     % \cmark & \cmark & 65.79 & 62.47 \\
%     \bottomrule
%     \end{tabular}
%     \label{table:ablation_pseudova}
% \end{table}

% \begin{figure*}[ht]
% \centering
% \begin{tabular}{cc}
% \subfloat{\includegraphics[width = 0.45\textwidth]{figs/ablation_neighbors_2.pdf}} 
% % & \subfloat{\includegraphics[width = 0.3\textwidth]{figs/ablation_threshold.pdf}}
% &
% \subfloat{\includegraphics[width = 0.45\textwidth]{figs/ablation_gamma_2.pdf}} 
% \end{tabular}
% \caption{Evaluation results with different numbers of neighbors (left) and values of $\gamma$ for regularization loss (right) on the RAF-DB dataset.}
% \label{fig:ablation_study}
% \end{figure*}

% ================================== Component analysis===================================

% ================================== Weighting Module===================================

% \begin{wrapfigure}{r}{0.5\textwidth}
% \vspace{-8ex}
%     \begin{center}
%       \includegraphics[width = 0.95\textwidth, height=0.8\textwidth]{figs/ablation_neighbors_2.pdf}
%     \end{center}
%     \caption{Evaluation results with different numbers of neighbors on the RAF-DB dataset.}
%     \label{fig:ablation_study}
%     \vspace{-3ex}
% \end{wrapfigure}

\textbf{Number of Nearest Neighbors.} We present the effect of the number of nearest neighbors $K$ on the model performance in Figure {\ref{fig:ablation_study}}. For original RAF-DB data, higher values of $K$ give better results but also require more training time. In particular, our training time with $K=8$ and $K=16$ on AffectNet is 12 hours and 20 hours respectively. Under noisy conditions, the best result is obtained with $K=8$ while larger or smaller $K$ can lead to slightly worse performance. The reason is that using a large $K$ might include more corrupted labels while using too few neighbors can limit the amount of exploitable information.

% \textbf{Minimum threshold for $b^i_k$} is a hyperparameter that controls the minimum contribution degree of each neighbor to the main instance. Figure {\ref{fig:ablation_study}} (middle) shows the network performance under different threshold values. When there is no threshold, the importance scores of the neighbors can be zero and we may lose some information about them, which hurts the accuracy of the model. On the other hand, a large threshold can lead to higher important scores on the noisy neighbors, which also decreases the model performance. We achieve the best result when the threshold is set to 0.2.}

% \textbf{Hyperparameter $\gamma$.} In Figure \ref{fig:ablation_study}, we investigate the hyperparameter $\gamma$ that controls the influence of the discriminative loss $\mathcal{L}_D$ in Equation \ref{eq:total_loss}. Overall, the performance on original data is not sensitive to the value of $\gamma$, and choosing $\gamma = 0.1$ achieves the best accuracy under both clean and noisy label condition.

% \begin{table}
% \centering
%     \setlength\aboverulesep{0pt}\setlength\belowrulesep{0pt}
%     \setcellgapes{3pt}\makegapedcells
    
%      \setlength{\tabcolsep}{6.5pt}  % Default value: 6pt
    
%     \caption{Test accuracy versus rejection rate results of different uncertainty learning methods on RAF-DB.\strut}
%     \begin{tabular}{l|cccc} 
%     \toprule
%     \multirow{2}{*}{Method} & \multicolumn{4}{c}{Accuracy (\%)} \\
% 	\cmidrule{2-5}
%      & 0\% rejection & 10\% rejection & 20\% rejection & 30\% rejection  \\ 
%     \midrule
%     \midrule

%     SCN \cite{scn} & 87.35 &	86.85 &	86.63 &	87.28 \\
%     DUL \cite{dul} & 88.04 &	90.11 &	92.58 &	94.50 \\
%     RUL \cite{rul} & 88.98 &	92.72 &	95.40 &	97.35 \\
    
%     \midrule
%     LDLVA (ours) & \textbf{89.57} &	\textbf{93.66} &	\textbf{96.5} &	\textbf{98.18} \\
%     \bottomrule
%     \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}
%     \end{tabular}%
%     \label{tab:accuracy_rejection_result}
% \end{table}
